Semantic Bounds and Strong Call-by-Value Normalization

This paper explores two topics at once: the use of denotational semantics to bound the evaluation length of functional programs, and the semantics of strong (that is, possibly under abstractions) call-by-value evaluation. About the first, we analyze de Carvalho's seminal use of relational semantics for bounding the evaluation length of lambda-terms, starting from the presentation of the semantics as an intersection types system. We focus on the part of his work which is usually neglected in its many recent adaptations, despite being probably the conceptually deeper one: how to transfer the bounding power from the type system to the relational semantics itself. We dissect this result and re-understand it via the isolation of a simpler size representation property. About the second, we use relational semantics to develop a semantical study of strong call-by-value evaluation, which is both a delicate and neglected topic. We give a semantic characterization of terms normalizable with respect to strong evaluation, providing in particular the first result of adequacy with respect to strong call-by-value. Moreover, we extract bounds about strong evaluation from both the type systems and the relational semantics. Essentially, we use strong call-by-value to revisit de Carvalho's semantic bounds, and de Carvalho's technique to provide semantical foundations for strong call-by-value.

==> 99-05-Normalization_and_Denotational_Semantics-proofs.tex <==
% !TEX root = main.tex
\section{Proofs of \Cref{SECT:NORMALIZATION}}

\begin{proposition}[Qualitative subjects + Stability by $\equiv$]
	\label{propappendix:qual-subject}
	\NoteState{prop:qual-subject}
	Let $\tm \tovsub \tm'$.
	\begin{enumerate}
		\item \label{pappendix:qual-subject-reduction}
		\emph{Reduction}: 	if $\namedtyjp{\tderiv}{}{\tm}{\typctx}{\mtype}$ then there is a derivation $\namedtyjp{\tderiv'}{}{\tm'}{\typctx}{\mtype}$ such that
		$\sizem{\tderiv'} \leq \sizem{\tderiv}$ and $\size{\tderiv'} \leq \size{\tderiv} $.
		
		\item \label{pappendix:qual-subject-expansion}
		\emph{Expansion}: if $\namedtyjp{\tderiv'}{}{\tm'}{\typctx}{\mtype}$ then there is a derivation $\namedtyjp{\tderiv}{}{\tm}{\typctx}{\mtype}$ such that
		$\sizem{\tderiv'} \leq \sizem{\tderiv}$ and $\size{\tderiv'} \leq \size{\tderiv} $.
		
		\item \label{pappendix:qual-subject-struct}
		\emph{Structural Equivalence}: if $\tm\eqstruct \tm'$ then $\namedtyjp{\tderiv}{}{\tm}{\typctx}{\mtype}$ if 
		and only if there is  $\namedtyjp{\tderiv'}{}{\tm'}{\typctx}{\mtype}$ with $\sizem{\tderiv} = \sizem{\tderiv'}$ 
		and $\size{\tderiv} = \size{\tderiv'} $.
	\end{enumerate}
\end{proposition}

\begin{proof}
	\begin{enumerate}
		\item By induction on	the evaluation context $\ctx$ in the step $\tm = \ctxp{\tmtwo} \tovsub \ctxp{\tmtwo'} = \tm'$ with $\tmtwo \rtom \tmtwo'$ or $\tmtwo' \rtoe \tmtwo'$. 
		The proof is analogous to the one for open quantitative subject reduction (\Cref{prop:weak-subject-reduction}), except that now there is one more case:
		\begin{itemize}
			\item \emph{Abstraction}, \ie $\ctx = \la{\var}{\ctxtwo}$. 
			Then, $\tm = \ctxp{\tmtwo} = \la{\var}{\ctxtwop{\tmtwo}} \allowbreak\rootRew{a} \la{\var}{\ctxtwop{\tmtwo'}} = \ctxp{\tmtwo'} = \tm'$ with $\tmtwo \rootRew{a} \tmtwo'$ and $a \in \{\msym, \esym\}$.
			Then, the derivation $\tderiv$ is necessarily (for some $n \in \nat$)
			\begin{equation*}
			\tderiv = 
			\begin{prooftree}[separation=1em]
%			\hypo{}
%			\ellipsis{$\tderivtwo_1$}{\typctx_1, \var \hastype \ptypetwo_1 \vdash \ctxtwop{\tmtwo} \hastype \ptypethree_1}
%			\infer1[\footnotesize$\lambda$]{\typctx_1 \vdash \la{\var}\ctxtwop{\tmtwo} \hastype \Pair{\ptypetwo_1}{\ptypethree_1}}
%			\hypo{\overset{n \in \nat}{\ldots}}
			\hypo{}
			\ellipsis{$\tderivtwo_i$}{\typctx_i, \var \hastype \mtypetwo_1 \vdash \ctxtwop{\tmtwo} \hastype \mtypethree_i}
			\infer1[\footnotesize$\lambda$]{\typctx_i \vdash \la{\var}\ctxtwop{\tmtwo} \hastype \larrow{\mtypetwo_i}{\mtypethree_i}}
			\delims{ \left( }{ \right)_{1 \leq i \leq n} }
			\infer1[\footnotesize$\ruleManyVal$]{\bigmplus_{i=1}^n \typctx_i \vdash \la{\var}\ctxtwop{\tmtwo} \hastype \bigmplus_{i=1}^{n} \mset{\larrow{\mtypetwo_i}{\mtypethree_i}} }
			\end{prooftree}
			\end{equation*}
			By \ih, for all $1 \leq i \leq n$, there is a derivation $\concl{\tderivtwo_i'}{\typctx_1, \var \hastype \mtypetwo_i}{\ctxtwop{\tmtwo'}}{\mtypethree_i}$ with: 
			$\size{\tderivtwo_i'} \leq \size{\tderivtwo_i}$ and $\sizem{\tderivtwo_i'} \leq \sizem{\tderivtwo_i}$.
			We can then build the derivation 
			\begin{equation*}
			\tderiv' = 
			\begin{prooftree}[separation=1em]
%			\hypo{}
%			\ellipsis{$\tderivtwo_1$}{\typctx_1, \var \hastype \ptypetwo_1 \vdash \ctxtwop{\tmtwo} \hastype \ptypethree_1}
%			\infer1[\footnotesize$\lambda$]{\typctx_1 \vdash \la{\var}\ctxtwop{\tmtwo} \hastype \Pair{\ptypetwo_1}{\ptypethree_1}}
%			\hypo{\overset{n \in \nat}{\ldots}}
			\hypo{}
			\ellipsis{$\tderivtwo'_i$}{\typctx_i, \var \hastype \mtypetwo_1 \vdash \ctxtwop{\tmtwop} \hastype \mtypethree_i}
			\infer1[\footnotesize$\lambda$]{\typctx_i \vdash \la{\var}\ctxtwop{\tmtwop} \hastype \larrow{\mtypetwo_i}{\mtypethree_i}}
			\delims{ \left( }{ \right)_{1 \leq i \leq n} }
			\infer1[\footnotesize$\ruleManyVal$]{\bigmplus_{i=1}^n \typctx_i \vdash \la{\var}\ctxtwop{\tmtwop} \hastype \bigmplus_{i=1}^{n} \mset{\larrow{\mtypetwo_i}{\mtypethree_i}} }
			\end{prooftree}
			\end{equation*}
			where
			\begin{enumerate}
				\item $\size{\tderiv'} = 1 + \sum_{i=1}^n \size{\tderivtwo_i'} \leq 1 + \sum_{i=1}^n \size{\tderivtwo_i} = \size{\tderiv}$ (note that $\size{\tderiv'} = \size{\tderiv}$ if $n = 0$); 
				\item $\sizem{\tderiv'} = \sum_{i=1}^n \sizem{\tderivtwo_i'} \leq  \sum_{i=1}^n \sizem{\tderivtwo_i} = \sizem{\tderiv}$ (note that $\sizem{\tderiv'} = \sizem{\tderiv}$ if $n = 0$).
			\end{enumerate}
		\end{itemize}
	
		\item By induction on	the evaluation context $\ctx$ in the step $\tm = \ctxp{\tmtwo} \tovsub \ctxp{\tmtwo'} = \tm'$ with $\tmtwo \rtom \tmtwo'$ or $\tmtwo' \rtoe \tmtwo'$. 
		The proof is analogous to the one for open quantitative subject expansion (\Cref{prop:weak-subject-expansion}), except that now there is one more case:
		\begin{itemize}
			\item \emph{Abstraction}, \ie $\ctx = \la{\var}{\ctxtwo}$. 
			Then, $\tm = \ctxp{\tmtwo} = \la{\var}{\ctxtwop{\tmtwo}} \allowbreak\rootRew{a} \la{\var}{\ctxtwop{\tmtwo'}} = \ctxp{\tmtwo'} = \tm'$ with $\tmtwo \rootRew{a} \tmtwo'$ and $a \in \{\msym, \esym\}$.
			Then, the derivation $\tderiv'$ is necessarily (for some $n \in \nat$)
			\begin{equation*}
			\tderiv' = 
			\begin{prooftree}[separation=1em]
%			\hypo{}
%			\ellipsis{$\tderivtwo_1$}{\typctx_1, \var \hastype \ptypetwo_1 \vdash \ctxtwop{\tmtwo} \hastype \ptypethree_1}
%			\infer1[\footnotesize$\lambda$]{\typctx_1 \vdash \la{\var}\ctxtwop{\tmtwo} \hastype \Pair{\ptypetwo_1}{\ptypethree_1}}
%			\hypo{\overset{n \in \nat}{\ldots}}
			\hypo{}
			\ellipsis{$\tderivtwo'_i$}{\typctx_i, \var \hastype \mtypetwo_1 \vdash \ctxtwop{\tmtwop} \hastype \mtypethree_i}
			\infer1[\footnotesize$\lambda$]{\typctx_i \vdash \la{\var}\ctxtwop{\tmtwop} \hastype \larrow{\mtypetwo_i}{\mtypethree_i}}
			\delims{ \left( }{ \right)_{1 \leq i \leq n} }
			\infer1[\footnotesize$\ruleManyVal$]{\bigmplus_{i=1}^n \typctx_i \vdash \la{\var}\ctxtwop{\tmtwop} \hastype \bigmplus_{i=1}^{n} \mset{\larrow{\mtypetwo_i}{\mtypethree_i}} }
			\end{prooftree}
			\end{equation*}
			By \ih, for all $1 \leq i \leq n$, there is a derivation $\concl{\tderivtwo_i}{\typctx_1, \var \hastype \mtypetwo_i}{\ctxtwop{\tmtwo}}{\mtypethree_i}$ with
			$\size{\tderivtwo_i'} \leq \size{\tderivtwo_i}$ and
			$\sizem{\tderivtwo_i'} \leq \sizem{\tderivtwo_i}$.
			We can then build the derivation 
			\begin{equation*}
			\tderiv = 
			\begin{prooftree}[separation=1em]
%			\hypo{}
%			\ellipsis{$\tderivtwo_1$}{\typctx_1, \var \hastype \ptypetwo_1 \vdash \ctxtwop{\tmtwo} \hastype \ptypethree_1}
%			\infer1[\footnotesize$\lambda$]{\typctx_1 \vdash \la{\var}\ctxtwop{\tmtwo} \hastype \Pair{\ptypetwo_1}{\ptypethree_1}}
%			\hypo{\overset{n \in \nat}{\ldots}}
			\hypo{}
			\ellipsis{$\tderivtwo_i$}{\typctx_i, \var \hastype \mtypetwo_1 \vdash \ctxtwop{\tmtwo} \hastype \mtypethree_i}
			\infer1[\footnotesize$\lambda$]{\typctx_i \vdash \la{\var}\ctxtwop{\tmtwo} \hastype \larrow{\mtypetwo_i}{\mtypethree_i}}
			\delims{ \left( }{ \right)_{1 \leq i \leq n} }
			\infer1[\footnotesize$\ruleManyVal$]{\bigmplus_{i=1}^n \typctx_i \vdash \la{\var}\ctxtwop{\tmtwo} \hastype \bigmplus_{i=1}^{n} \mset{\larrow{\mtypetwo_i}{\mtypethree_i}} }
			\end{prooftree}
			\end{equation*}
			where
			\begin{enumerate}
				\item $\size{\tderiv} = 1 + \sum_{i=1}^n \size{\tderivtwo_i} \leq 1 + \sum_{i=1}^n \size{\tderivtwo_i'} = \size{\tderiv'}$ (note that $\size{\tderiv'} = \size{\tderiv}$ if $n = 0$); 
				\item $\sizem{\tderiv} = \sum_{i=1}^n \sizem{\tderivtwo_i} \leq  \sum_{i=1}^n \sizem{\tderivtwo_i'} = \sizem{\tderiv'}$ (note that $\sizem{\tderiv'} = \sizem{\tderiv}$ if $n = 0$).

			\end{enumerate}
		\end{itemize} 
	
		\item By structural induction on the context $\ctx$ such that $\tm = \ctxp{\tmtwo} \eqstruct \ctxp{\tmtwop} = \tmp$. In each case, the proof that $\size{\tderiv} = \size{\tderivp}$ and $\sizem{\tderiv} = \sizem{\tderivp}$ is rather evident, and so will not be explicitly explained. By symmetry of $\equiv$, it is enough to prove only one implication of the equivalence.
		\begin{itemize}
			\item \emph{Empty context}; \ie, $\ctx = \ctxhole$. There are several sub-cases to this:
			\begin{itemize}
				\item Let $\tm = \tmtwo = \tmthree \esub{\vartwo}{\tmfour} \esub{\varthree}{\tmfive} \tostructcom \tmthree \esub{\varthree}{\tmfive} \esub{\vartwo}{\tmfour} = \tmtwop = \tmp$, with $\vartwo \notin \fv{\tmfive}$ and $\varthree \notin \fv{\tmfour}$. Then $\tderiv$ is of the form	
				\begin{prooftree*}
					\hypo{}
					\ellipsis{$\tderivtwo$}{\tyjp{}{\tmthree}{\typctxtwo, \vartwo \hastype \mtypetwo ; \varthree \hastype \mtypethree}{\mtype}}
					\hypo{}
					\ellipsis{$\tderivthree$}{\tyjp{}{\tmfour}{\typctxthree}{\mtypetwo}}
					\infer2[\footnotesize$\ruleES$]{\tyjp{}{\tmthree \esub{\vartwo}{\tmfour}}{\typctxtwo \mplus \typctxthree, \varthree \hastype \mtypethree}{\mtype}}
					\hypo{}
					\ellipsis{$\tderivfour$}{\tyjp{}{\tmfive}{\typctxfour}{\mtypethree}}
					\infer2[\footnotesize$\ruleES$]{\tyjp{}{\tmthree \esub{\vartwo}{\tmfour} \esub{\varthree}{\tmfive}}{\typctxtwo \mplus \typctxthree \mplus \typctxfour}{\mtype}}
				\end{prooftree*}
				
				noting that since $\vartwo \notin \fv{\tmfive}$ and $\varthree \notin \fv{\tmfour}$ then $\vartwo \notin \dom{\typctxfour}$ and $\varthree \notin \dom{\typctxthree}$ ---by \refrmk{free-variables}. Thus, we can derive $\tderivp$ as
				
				\begin{prooftree*}
					\hypo{}
					\ellipsis{$\tderivtwo$}{\tyjp{}{\tmthree}{\typctxtwo, \vartwo \hastype \mtypetwo ; \varthree \hastype \mtypethree}{\mtype}}
					\hypo{}
					\ellipsis{$\tderivfour$}{\tyjp{}{\tmfive}{\typctxfour}{\mtypethree}}
					\infer2[\footnotesize$\ruleES$]{\tyjp{}{\tmthree \esub{\varthree}{\tmfive}}{\typctxtwo \mplus \typctxfour, \vartwo \hastype \mtypetwo}{\mtype}}
					\hypo{}
					\ellipsis{$\tderivthree$}{\tyjp{}{\tmfour}{\typctxthree}{\mtypetwo}}
					\infer2[\footnotesize$\ruleES$]{\tyjp{}{\tmthree \esub{\varthree}{\tmfive} \esub{\vartwo}{\tmfour}}{\typctxtwo \mplus \typctxthree \mplus \typctxfour}{\mtype}}
				\end{prooftree*}
				
				\item Let $\tm = \tmtwo = \tmthree (\tmfour \esub{\vartwo}{\tmfive}) \tostructapr (\tmthree \tmfour) \esub{\vartwo}{\tmfive} = \tmtwop = \tmp$, with $\vartwo \notin \fv{\tmthree}$. Then $\tderiv$ is of the form
				
				\begin{prooftree*}
					\hypo{}
					\ellipsis{$\tderivtwo$}{\tyjp{}{\tmthree}{\typctxtwo}{\mult{\ty{\mtypetwo}{\mtype}}}}
					\hypo{}
					\ellipsis{$\tderivthree$}{\tyjp{}{\tmfour}{\typctxthree, \vartwo \hastype \mtypethree}{\mtypetwo}}
					\hypo{}
					\ellipsis{$\tderivfour$}{\tyjp{}{\tmfive}{\typctxfour}{\mtypethree}}
					\infer2[\footnotesize$\ruleES$]{\tyjp{}{\tmfour \esub{\vartwo}{\tmfive}}{\typctxthree \mplus \typctxfour}{\mtypetwo}}
					\infer2[\footnotesize$\ruleApp$]{\tyjp{}{\tmthree (\tmfour \esub{\vartwo}{\tmfive})}{\typctxtwo \mplus \typctxthree \mplus \typctxfour}{\mtype}}
				\end{prooftree*}
				
				noting that $\vartwo \notin \dom{\typctxtwo}$ ---by \refrmk{free-variables}. Thus, we can derive $\tderivp$ as 
				
				\begin{prooftree*}
					\hypo{}
					\ellipsis{$\tderivtwo$}{\tyjp{}{\tmthree}{\typctxtwo}{\mult{\ty{\mtypetwo}{\mtype}}}}
					\hypo{}
					\ellipsis{$\tderivfour$}{\tyjp{}{\tmfour}{\typctxthree, \vartwo \hastype \mtypethree}{\mtypetwo}}
					\infer2[\footnotesize$\ruleApp$]{\tyjp{}{\tmthree \tmfour}{\typctxtwo \mplus \typctxthree, \vartwo \hastype \mtypethree}{\mtype}}
					\hypo{}
					\ellipsis{$\tderivthree$}{\tyjp{}{\tmfive}{\typctxfour}{\mtypethree}}
					\infer2[\footnotesize$\ruleES$]{\tyjp{}{(\tmthree \tmfour) \esub{\vartwo}{\tmfive}}{\typctxtwo \mplus \typctxfour \mplus \typctxthree}{\mtype}}
				\end{prooftree*}
				
				\item The case where $\tm = \tmtwo = (\tmthree \tmfour) \esub{\vartwo}{\tmfive} \tostructapr \tmthree (\tmfour \esub{\vartwo}{\tmfive}) = \tmtwop = \tmp$, with $\vartwo \notin \fv{\tmthree}$, follows a similar reasoning to the previous case and is left for the reader.
				
				\item Let $\tm = \tmtwo = (\tmthree \esub{\vartwo}{\tmfour}) \tmfive \tostructapl (\tmthree \tmfive) \esub{\vartwo}{\tmfour} = \tmtwop = \tmp$, with $\vartwo \notin \fv{\tmfive}$. Then $\tderiv$ is of the form
				
				\begin{prooftree*}
					\hypo{}
					\ellipsis{$\tderivtwo$}{\tyjp{}{\tmthree}{\typctxtwo, \vartwo \hastype \mtypethree}{\mult{\ty{\mtypetwo}{\mtype}}}}
					\hypo{}
					\ellipsis{$\tderivthree$}{\tyjp{}{\tmfour}{\typctxthree}{\mtypethree}}
					\infer2[\footnotesize$\ruleES$]{\tyjp{}{\tmthree \esub{\vartwo}{\tmfour}}{\typctxtwo \mplus \typctxthree}{\mult{\ty{\mtypetwo}{\mtype}}}}
					\hypo{}
					\ellipsis{$\tderivfour$}{\tyjp{}{\tmfive}{\typctxfour}{\mtypetwo}}
					\infer2[\footnotesize$\ruleApp$]{\tyjp{}{(\tmthree \esub{\vartwo}{\tmfour}) \tmfive}{\typctxtwo \mplus \typctxthree \mplus \typctxfour}{\mtype}}
				\end{prooftree*}
				
				noting that $\vartwo \notin \dom{\typctxfour}$ ---by \refrmk{free-variables}. Thus, we can derive $\tderivp$ as 
				
				\begin{prooftree*}
					\hypo{}
					\ellipsis{$\tderivtwo$}{\tyjp{}{\tmthree}{\typctxtwo, \vartwo \hastype \mtypethree}{\mult{\ty{\mtypetwo}{\mtype}}}}
					\hypo{}
					\ellipsis{$\tderivfour$}{\tyjp{}{\tmfive}{\typctxfour}{\mtypetwo}}
					\infer2[\footnotesize$\ruleApp$]{\tyjp{}{\tmthree \tmfive}{\typctxtwo \mplus \typctxfour, \vartwo \hastype \mtypethree}{\mtype}}
					\hypo{}
					\ellipsis{$\tderivfour$}{\tyjp{}{\tmfour}{\typctxthree}{\mtypethree}}
					\infer2[\footnotesize$\ruleES$]{\tyjp{}{(\tmthree \tmfive) \esub{\vartwo}{\tmfour}}{\typctxtwo \mplus \typctxthree \mplus \typctxfour}{\mtype}}
				\end{prooftree*}
				
				\item The case where $\tm = \tmtwo = (\tmthree \tmfive) \esub{\vartwo}{\tmfour} \tostructapl (\tmthree \esub{\vartwo}{\tmfour}) \tmfive = \tmtwop = \tmp$, with $\vartwo \notin \fv{\tmfive}$, follows a similar reasoning to the previous case and is left for the reader.
				
				\item Let $\tm = \tmtwo = \tmthree \esub{\vartwo}{\tmfour \esub{\varthree}{\tmfive}} \tostructes \tmtwo \esub{\vartwo}{\tmfour} \esub{\varthree}{\tmfive} = \tmtwop = \tmp$, with $\varthree \notin \fv{\tmthree}$. Then $\tderiv$ is of the form
				
				\begin{prooftree*}
					\hypo{}
					\ellipsis{$\tderivtwo$}{\tyjp{}{\tmthree}{\typctxtwo, \vartwo \hastype \mtypetwo}{\mtype}}
					\hypo{}
					\ellipsis{$\tderivthree$}{\tyjp{}{\tmfour}{\typctxthree, \varthree \hastype \mtypethree}{\mtypetwo}}
					\hypo{}
					\ellipsis{$\tderivfour$}{\tyjp{}{\tmfive}{\typctxfour}{\mtypethree}}
					\infer2[\footnotesize$\ruleES$]{\tyjp{}{\tmfour \esub{\varthree}{\tmfive}}{\typctxthree \mplus \typctxfour}{\mtypetwo}}
					\infer2[\footnotesize$\ruleES$]{\tyjp{}{\tmthree \esub{\vartwo}{\tmfour \esub{\varthree}{\tmfive}}}{\typctxtwo \mplus \typctxthree \mplus \typctxfour}{\mtype}}
				\end{prooftree*}
				
				noting that $\varthree \notin \dom{\typctxtwo}$ ---by \refrmk{free-variables}. Thus, we can derive $\tderivp$ as 
				
				\begin{prooftree*}
					\hypo{}
					\ellipsis{$\tderivtwo$}{\tyjp{}{\tmthree}{\typctxtwo, \vartwo \hastype \mtypetwo}{\mtype}}
					\hypo{}
					\ellipsis{$\tderivthree$}{\tyjp{}{\tmfour}{\typctxthree, \varthree \hastype \mtypethree}{\mtypetwo}}
					\infer2[\footnotesize$\ruleES$]{\tyjp{}{\tmthree \esub{\vartwo}{\tmfour}}{\typctxtwo \mplus \typctxthree, \varthree \hastype \mtypethree}{\mtype}}
					\hypo{}
					\ellipsis{$\tderivfour$}{\tyjp{}{\tmfive}{\typctxfour}{\mtypethree}}
					\infer2[\footnotesize$\ruleES$]{\tyjp{}{\tmthree \esub{\vartwo}{\tmfour} \esub{\varthree}{\tmfive}}{\typctxtwo \mplus \typctxthree \mplus \typctxfour}{\mtype}}
				\end{prooftree*}
				
				\item The case where $\tm = \tmtwo = \tmtwo \esub{\vartwo}{\tmfour} \esub{\varthree}{\tmfive} \tostructes \tmthree \esub{\vartwo}{\tmfour \esub{\varthree}{\tmfive}} = \tmtwop = \tmp$, with $\varthree \notin \fv{\tmthree}$, follows a similar reasoning to the previous case and is left for the reader.
				
			\end{itemize}
			
			\item \emph{Application right}; \ie, $\ctx = \tmthree \ctxtwo$. Then $\tm = \tmthree \ctxtwop{\tmtwo} \eqstruct \tmthree \ctxtwop{\tmtwop} = \tmp$, and $\tderiv$ is of the form
			
			\begin{prooftree*}
				\hypo{}
				\ellipsis{$\tderivtwo$}{\tyjp{}{\tmthree}{\typctxtwo}{\mult{\ty{\mtypetwo}{\mtype}}}}
				\hypo{}
				\ellipsis{$\tderivthree$}{\tyjp{}{\ctxtwop{\tmtwo}}{\typctxthree}{\mtypetwo}}
				\infer2[\footnotesize$\ruleApp$]{\tyjp{}{\tmthree \ctxtwop{\tmtwo}}{\typctxtwo \mplus \typctxthree}{\mtype}}
			\end{prooftree*}
			
			By \ih on $\ctxtwop{\tmtwo}$ and $\tderivthree$, there exists $\namedtyjp{\tderivthreep}{}{\ctxtwop{\tmtwop}}{\typctxthree}{\mtypetwo}$. Thus, we can derive $\tderivp$ as follows
			
			\begin{prooftree*}
				\hypo{}
				\ellipsis{$\tderivtwo$}{\tyjp{}{\tmthree}{\typctxtwo}{\mult{\ty{\mtypetwo}{\mtype}}}}
				\hypo{}
				\ellipsis{$\tderivthreep$}{\tyjp{}{\ctxtwop{\tmtwop}}{\typctxthree}{\mtypetwo}}
				\infer2[\footnotesize$\ruleApp$]{\tyjp{}{\tmthree \ctxtwop{\tmtwop}}{\typctxtwo \mplus \typctxthree}{\mtype}}
			\end{prooftree*}
			
			\item \emph{Application left}; \ie, $\ctx = \ctxtwo \tmthree$. Then $\tm = \ctxtwop{\tmtwo} \tmthree \eqstruct \ctxtwop{\tmtwop} \tmthree = \tmp$, and $\tderiv$ is of the form
			
			\begin{prooftree*}
				\hypo{}
				\ellipsis{$\tderivtwo$}{\tyjp{}{\ctxtwop{\tmtwo}}{\typctxtwo}{\mult{\ty{\mtypetwo}{\mtype}}}}
				\hypo{}
				\ellipsis{$\tderivthree$}{\tyjp{}{\tmthree}{\typctxthree}{\mtypetwo}}
				\infer2[\footnotesize$\ruleApp$]{\tyjp{}{\ctxtwop{\tmtwo} \tmthree}{\typctxtwo \mplus \typctxthree}{\mtype}}
			\end{prooftree*}
			
			By \ih on $\ctxtwop{\tmtwo}$ and $\tderivtwo$, there exists $\namedtyjp{\tderivtwop}{}{\ctxtwop{\tmtwop}}{\typctxtwo}{\mult{\ty{\mtypetwo}{\mtype}}}$. Thus, we can derive $\tderivp$ as follows
			
			\begin{prooftree*}
				\hypo{}
				\ellipsis{$\tderivtwop$}{\tyjp{}{\ctxtwop{\tmtwop}}{\typctxtwo}{\mult{\ty{\mtypetwo}{\mtype}}}}
				\hypo{}
				\ellipsis{$\tderivthree$}{\tyjp{}{\tmthree}{\typctxthree}{\mtypetwo}}
				\infer2[\footnotesize$\ruleApp$]{\tyjp{}{\ctxtwop{\tmtwop} \tmthree}{\typctxtwo \mplus \typctxthree}{\mtype}}
			\end{prooftree*}
			
			\item \emph{Under $\lambda$-abstraction}; \ie, $\ctx = \la{\var}{\ctxtwo}$. Then $\tm = \la{\var}{\ctxtwop{\tmtwo}} \eqstruct \la{\var}{\ctxtwop{\tmtwop}} = \tmp$ and $\tderiv$ is of the form
			
			\begin{prooftree*}
				\hypo{}
				\ellipsis{$\tderiv_{i}$}{\tyjp{}{\ctxtwop{\tmtwo}}{\typctx_{i}, \var \hastype \mtypethree_{i}}{\mtypetwo_{i}}}
				\infer1[\footnotesize$\ruleFun$]{\tyjp{}{\la{\var}{\ctxtwop{\tmtwo}}}{\typctx_{i}}{\mult{\ty{\mtypethree_{i}}{\mtypetwo_{i}}}}}
				\delims{ \left( }{ \right)_{\iI} }
				\infer1[\footnotesize$\ruleES$]{\tyjp{}{\la{\var}{\ctxtwop{\tmtwo}}}{\bigmplus_{i=1}^{n} \typctx_{i}}{\bigmplus_{i=1}^{n} \mult{\ty{\mtypethree_{i}}{\mtypetwo_{i}}}}}
			\end{prooftree*}
			
			By \ih on $\ctxtwop{\tmtwo}$ and $\tderiv_{i}$, for each $\iI$, there exists $\namedtyjp{\tderivp_{i}}{}{\ctxtwop{\tmtwop}}{\typctx_{i} ; \var \hastype \mtypethree_{i}}{\mtypetwo_{i}}$. Thus, we can derive $\tderivp$ as follows
			
			\begin{prooftree*}
				\hypo{}
				\ellipsis{$\tderivp_{i}$}{\tyjp{}{\ctxtwop{\tmtwop}}{\typctx_{i}, \var \hastype \mtypethree_{i}}{\mtypetwo_{i}}}
				\infer1[\footnotesize$\ruleFun$]{\tyjp{}{\la{\var}{\ctxtwop{\tmtwop}}}{\typctx_{i}}{\mult{\ty{\mtypethree_{i}}{\mtypetwo_{i}}}}}
				\delims{ \left( }{ \right)_{\iI} }
				\infer1[\footnotesize$\ruleES$]{\tyjp{}{\la{\var}{\ctxtwop{\tmtwop}}}{\bigmplus_{i=1}^{n} \typctx_{i}}{\bigmplus_{i=1}^{n} \mult{\ty{\mtypethree_{i}}{\mtypetwo_{i}}}}}
			\end{prooftree*}
			
			\item \emph{$\mathsf{ES}$ right}; \ie, $\ctx = \tmthree \esub{\var}{\ctxtwo}$. Then $\tm = \tmthree \esub{\var}{\ctxtwop{\tmtwo}} \eqstruct \tmthree \esub{\var}{\ctxtwop{\tmtwop}} = \tmp$ and $\tderiv$ is of the form
			
			\begin{prooftree*}
				\hypo{}
				\ellipsis{$\tderivtwo$}{\tyjp{}{\tmthree}{\typctxtwo, \var \hastype \mtypetwo}{\mtype}}
				\hypo{}
				\ellipsis{$\tderivthree$}{\tyjp{}{\ctxtwop{\tmtwo}}{\typctxthree}{\mtypetwo}}
				\infer2[\footnotesize$\ruleES$]{\tyjp{}{\tmthree \esub{\var}{\ctxtwop{\tmtwo}}}{\typctxtwo \mplus \typctxthree}{\mtype}}
			\end{prooftree*}
			
			By \ih on $\ctxtwop{\tmtwo}$ and $\tderivthree$, there exists $\namedtyjp{\tderivthreep}{}{\ctxtwop{\tmtwop}}{\typctxthree}{\mtypetwo}$. Thus, we can derive $\tderivp$ as follows
			
			\begin{prooftree*}
				\hypo{}
				\ellipsis{$\tderivtwo$}{\tyjp{}{\tmthree}{\typctxtwo, \var \hastype \mtypetwo}{\mtype}}
				\hypo{}
				\ellipsis{$\tderivthreep$}{\tyjp{}{\ctxtwop{\tmtwop}}{\typctxthree}{\mtypetwo}}
				\infer2[\footnotesize$\ruleES$]{\tyjp{}{\tmthree \esub{\var}{\ctxtwop{\tmtwo}}}{\typctxtwo \mplus \typctxthree}{\mtype}}
			\end{prooftree*}
			
			\item \emph{$\mathsf{ES}$ left}; \ie, $\ctx = \ctxtwo \esub{\var}{\tmthree }$. Then $\tm = \ctxtwop{\tmtwo} \esub{\var}{\tmthree} \eqstruct \ctxtwop{\tmtwo} \esub{\var}{\tmthree} = \tmp$ and $\tderiv$ is of the form
			
			\begin{prooftree*}
				\hypo{}
				\ellipsis{$\tderivtwo$}{\tyjp{}{\ctxtwop{\tmtwo}}{\typctxtwo, \var \hastype \mtypetwo}{\mtype}}
				\hypo{}
				\ellipsis{$\tderivthree$}{\tyjp{}{\tmthree}{\typctxthree}{\mtypetwo}}
				\infer2[\footnotesize$\ruleES$]{\tyjp{}{\ctxtwop{\tmtwo} \esub{\var}{\tmthree}}{\typctxtwo \mplus \typctxthree}{\mtype}}
			\end{prooftree*}
			
			By \ih on $\ctxtwop{\tmtwo}$ and $\tderivtwo$, there exists $\namedtyjp{\tderivtwop}{}{\ctxtwop{\tmtwop}}{\typctxtwo ; \var \hastype \mtypetwo}{\mtype}$. Thus, we can derive $\tderivp$ as follows
			
			\begin{prooftree*}
				\hypo{}
				\ellipsis{$\tderivtwop$}{\tyjp{}{\ctxtwop{\tmtwop}}{\typctxtwo, \var \hastype \mtypetwo}{\mtype}}
				\hypo{}
				\ellipsis{$\tderivthree$}{\tyjp{}{\tmthree}{\typctxthree}{\mtypetwo}}
				\infer2[\footnotesize$\ruleES$]{\tyjp{}{\ctxtwop{\tmtwo} \esub{\var}{\tmthree}}{\typctxtwo \mplus \typctxthree}{\mtype}}
			\end{prooftree*}
			
		\end{itemize}
		\qedhere
	\end{enumerate}
\end{proof}

Point 3 prove that typability in the theory of the VSC is considered up to structural equivalence between terms. Note that the size of type derivations is also preserved via structural equivalence; this is a crucial point regarding bounds (and in particular \emph{minimal bounds}) in the size of type derivations for $\vsubterms$ modulo structural equivalence.


%\begin{theorem}[$\tovsubs$ is normalizing]
%	\label{thmappendix:normalization}
%	\NoteState{thm:normalization}
%	Let $\tm \tovsub^* \tmtwo$ be an evaluation to normal form. Then $\tm \tovsubs^* \tmtwo$.
%\end{theorem}
%
%\begin{proof}
%	\refprop{typability-normal} gives a unitary shrinking type derivation $\concl{\tderiv}{\typctx}{\tmtwo}{\ptype}$ for $\tmtwo$. Qualitative subject expansion (\refpropp{qual-subject}{expansion}) iterated along $\tm \tovsub^* \tmtwo$ gives a unitary shrinking derivation $\concl{\tderivtwo}{\typctx}{\tm}{\ptype}$ for $\tm$. Quantitative correctness (\refthm{correctness}) implies $\tm \tovsubs^* \tmthree$ with $\tmthree$ normal. Confluence gives $\tmthree = \tmtwo$.
%\end{proof}





==> 99-06-Fireballs-proofs.tex <==
% !TEX root = main.tex
\section{Proofs of \Cref{SECT:FIREBALLS}}
\label{app:fireballs-proofs}

\paragraph{The Strong Fireball Calculus is Not Confluent} Before studying the properties of strong evaluation for 
call-by-fireball $\beta$-reduction, let us see why the \emph{strong} fireball calculus is not confluent.
For any $\Rule \in \{\betaabs,\betain\}$, let $\torule$ be the closure of $\rootRew{\Rule}$ (defined on 
p.~\pageref{SECT:FIREBALLS}) under \emph{any} evaluation context $\ctx$, and let strong fireball \emph{reduction} be 
$\tof \defeq \tobabs \cup \toin$.
To show that $\tof$ is not confluent, consider the term $\tm \defeq (\la{\vartwo}I(\vartwo\vartwo))\delta$, where $I = 
\la{\varthree}{\varthree}$ and $\delta \defeq \la{\varthree}\varthree\varthree$: then, $\tm \tobabs I({\delta\delta})$ 
which can only reduce to itself (note that ${\delta\delta}$ is neither a value nor an inert term), but $\tm \toin 
(\la{\vartwo}\varthree \esub{\varthree}{\vartwo\vartwo})\delta$ which cannot reduce to $I({\delta\delta})$.
The problem here is that the step $\toin$ is somehow ``wrong'' because the argument $\vartwo\vartwo$ of the internal 
$\betain$-redex is not a ``real'' inert term: indeed, it is inside an external $\betaabs$-redex binding the variable 
$\vartwo$ to the value $\delta$, and  the step $\tobabs$ transforms it in a term that is no longer a fireball.

The deep reason for the lack of confluence is that fireballs are not closed under substitution, indeed substituting a 
value for a variable in a inert term might yield a term that is not a variable, for instance $(\vartwo\vartwo) 
\isub{\vartwo}{\delta} = \delta\delta$ in the example above. 
This problem is avoided by the strong fireball \emph{strategy} $\tofs$ defined on p.~\pageref{SECT:FIREBALLS} because it 
ensures that %the function part of 
a fired $\betaf$-redex does not contain any other $\betaf$-redex that it can fire.

\paragraph{About Light Terms} Some considerations before proving that lightness is preserved by strong fireball 
strategy $\tofs$.
We say that a context $\ctx$ is \emph{\sopen} if $\ctx = \strongctxp{\openctx}$ for some strong context $\strongctx$ and 
some open context $\openctx$.
Note that, according to the definition of strong fireball strategy, for $\Rule \in \{\betaabs, \betain\}$, $\tm 
\Rew{\esssym\Rule} \tm'$ means that $\tm = \strongctxp{\openctxp{\tmtwo}}$ and $\tm' = \strongctxp{\openctxp{\tmtwo'}}$ 
with $\tmtwo \rootRew{\Rule} \tmtwo'$, for some \sopen context $\strongctxp{\openctx}$.
Below, we implicitly use the fact that all inert terms are rigid.

Lightness is a quite delicate, unhandy notion.
First, note that lightness cannot be proved by mere induction on terms.
Indeed, $\la{\var}\var\esub{\varthree}{\itm}$ and $\vartwo$ and $\la{\vartwo}{\vartwo}$ are light but $(\la{\var}\var 
\esub{\varthree}{\itm})\vartwo$ and $(\la{\vartwo}{\vartwo}) \la{\var}\var \esub{\varthree}{\itm}$ are not (since 
$(\la{\var}\ctxhole)\vartwo$ and $(\la{\vartwo}\vartwo)\la{\var}\ctxhole$ are not \sopen-contexts). 
The fact that the left and right subterms of an application are light is not enough to conclude that the application 
itself is light.

Besides, lightness is not even preserved by substitution: $\la{\var}(\var\esub{\varthree}{\itm})$ and $\var\vartwo$ and 
$\var \, \la{\var}(\var \esub{\varthree}{\itm})$ are light, but \allowbreak$(\var\vartwo)\isub{\var}{\la{\var}(\var 
\esub{\varthree}{\itm})} = (\la{\var}(\var \esub{\varthree}{\itm}))\vartwo$ and \allowbreak $(\var \, \la{\var}(\var 
\esub{\varthree}{\itm} ))\isub{\var}{\la{\vartwo}\vartwo} = (\la{\vartwo}{\vartwo}) \la{\var}(\var 
\esub{\varthree}{\itm})$ are not, as we have just seen.
 
Finally, lightness is not preserved by strong fireball reduction $\tof$.
Indeed $(\la{\var}(\la{\varthree} \var ){\itm})\vartwo$ is light, since there are no \ES, but $(\la{\var}(\la{\varthree} 
\var ){\itm})\vartwo \tof (\la{\var}(\var \esub{\varthree}{\itm}))\vartwo$ which is not light.
Note that strong fireball strategy $\tofs$ cannot fire the internal $\betain$-redex $(\la{\varthree} \var ){\itm}$, in 
fact it fires the external $\betaf$-redex: $(\la{\var}(\la{\varthree} \var ){\itm})\vartwo \tofs ((\la{\varthree} \var 
){\itm})\esub{\var}{\vartwo}$ which is still light. 

Light terms enjoy the following property.

\begin{lemma}[No \ES inside $\betaf$-redexes]
	\label{l:no-es}
	Let $\tm$ be a light term.
	\begin{enumerate}
		\item\label{p:no-es-base} If $\tm = \sctxp{\la{\var}\tmtwo}\sctxtwop{\tmthree}$ then $\tmtwo$ and $\tmthree$ are 
without \ES.
		\item\label{p:no-es-so} If $\tm = \strongctxp{\openctxp{\sctxp{\la{\var}\tmtwo}\sctxtwop{\tmthree}}}$ then $\tmtwo$ 
and $\tmthree$ are without \ES.
	\end{enumerate} 
\end{lemma}	

\begin{proof}
	\begin{enumerate}
		\item  The terms $\tmtwo$ and $\tmthree$ are without \ES. Indeed:
		\begin{itemize}
			\item if $\tmtwo$ had some \ES then $\tmtwo = \strongctxp{\openctxp{\tmfour \esub{\varthree}{\itm}}}$ by 
lightness, but $\tm$ would not be light because $\subctxp{\la{\var}{\strongctxp{\openctx}}} \subctxtwop{\tmthree}$ is 
not a \sopen context;
			\item if $\tmthree$ had some \ES then $\tmthree = \la{\vartwo}\strongctxp{\openctxp{\tmfour 
\esub{\varthree}{\itm}}}$ by lightness, but $\tm$ would not be light because $\subctxp{\la{\var}{\tmtwo}} 
\subctxtwop{\la{\vartwo}\strongctx}$ is not a \sopen context.
		\end{itemize}
		\item By induction on the definition of strong context $\strongctx$ and open context $\openctx$.
		The base case $\strongctx = \ctxhole = \openctx$ is \Cref{p:no-es-base} above, the other cases follow from the \ih 
smoothly. 
		\qedhere 
	\end{enumerate}
\end{proof}

\Cref{l:no-es}.\ref{p:no-es-so} means that, in a light term, the function and argument parts of any $\betaf$-redex that 
can be fired by strong fireball strategy $\tofs$ do not contain any \ES.
Thus, when strong fireball strategy fires a $\betaabs$-redex in a light term, inert terms in \ES cannot be transformed 
in non-inert terms, circumventing the aforementioned problem that substituting a value in a inert term may yield a 
non-inert term. 
This property is crucial to prove that lightness is preserved by strong fireball strategy $\tofs$, and shows why it is 
important that in a light term not only all \ES only contain inert terms, but also they are located in a \sopen context, 
so that they are not inside an external $\betaabs$-redex that can be fired by $\tofs$.

\begin{lemma}[Preservations]
	\label{l:preservation-light}
	Let $\tm$ be a term and $\val$ be a value.
	\begin{enumerate}
		\item\label{p:preservation-light-substitution} \emph{Substitution:} %For any value $\val$, 
		If $\tm$ and $\val$ are without \ES, then $\tm \isub{\var}{\val}$ is without \ES.
		\item\label{p:preservation-light-reduction} \emph{Strong strategy:} 	If $\tm$ is light and $\tm \tofs \tm'$ then 
$\tm'$ is light.
	\end{enumerate}
\end{lemma}

\begin{proof}\hfill
	\begin{enumerate}
		\item By induction $\tm$.
		Cases:
		\begin{itemize}
			\item \emph{Variable}, \ie $\tm = \vartwo$.
			If $\vartwo = \var$ then $\tm\isub{\var}{\val} = \val$, which is without \ES by hypothesis.
			Otherwise, $\vartwo \neq \var$ and then $\tm\isub{\var}{\val} = \vartwo$, which is without \ES.
			
			\item \emph{Application}, \ie $\tm = \tmtwo \tmthree$.
			By \ih, $\tmtwo\isub{\var}{\val}$ and $\tmthree\isub{\var}{\val}$ are without \ES. 
			Therefore,  $\tm\isub{\var}{\val} = \tmtwo\isub{\var}{\val}\tmthree\isub{\var}{\val}$ is without \ES. 
			
			\item \emph{Abstraction}, \ie $\tm = \la{\vartwo}\tmtwo$, and we can suppose without loss of generality that 
$\vartwo \notin \fv{\val} \cup \{\var\}$.
			By \ih, $\tmtwo \isub{\var}{\val}$ is without \ES and therefore $\tm\isub{\var}{\val} = \la{\vartwo}\tmtwo 
\isub{\var}{\val}$ is without \ES.
			
			\item \emph{Explicit substitution}, \ie $\tm = \tmtwo\esub{\vartwo}{\tmthree}$. 
			This case is impossible because $\tm$ is without \ES by hypothesis.
			
		\end{itemize}
		
		\item Two cases, depending on whether $\tm \tobetavs \tm'$ or  $\tm \toins \tm'$.
		\begin{itemize}
			\item \emph{Value step}: If $\tm \tobetavs \tm'$ then $\tm = \strongctxp{\openctxp{ \sctxp{\la{\var}\tmtwo} 
\sctxtwop{\val}}}$ and $\tm' = \strongctxp{\openctxp{\sctxtwop{\sctxp{{\tmtwo}\isub{\var}{\val}}} }}$.
			As $\tm$ is light, $\tmtwo$ and $\val$ are without \ES by \Cref{l:no-es}.\ref{p:no-es-so}.
			By \reflemmap{preservation-light}{substitution}, ${\tmtwo}\isub{\var}{\val}$ is without \ES.
			Therefore, $\tm'$ is light.
			\item \emph{Inert step}: If $\tm \toins \tm'$ then $\tm = \strongctxp{\openctxp{ \sctxp{\la{\var}\tmtwo} \itm }}$ 
and $\tm' = \strongctxp{\openctxp{\sctxp{{\tmtwo}\esub{\var}{\itm}} }}$.
			As $\tm$ is light, $\tmtwo$ is without \ES and $\itm = \sctxtwop{\itmtwo}$ with $\itm'$ without \ES, by 
\Cref{l:no-es}.\ref{p:no-es-so}.
						Therefore, $\tm'$ is light.
			\qedhere
		\end{itemize}
	\end{enumerate}
\end{proof}



\begin{proposition}
	\label{propappendix:props-of-tofs}
	Let $\tm$ be a light term.
	\NoteState{prop:props-of-tofs}
	\begin{enumerate}
		\item \emph{Simulation}:\label{pappendix:props-of-tofs-simulation} if $\deriv:\tm\tofs^* \tmtwo$ then there is 
$\derivp:\tm\tovsubvals^{\leq 2\size\deriv} \tmtwo$ with $\size\deriv = \sizem\derivp$.
		\item \emph{Harmony}: $\tm$ is $\tofs$ normal iff it is a strong fireball.
		
		\item \label{pappendix:props-of-tofs-diamond} \emph{Diamond}: $\tofs$ is diamond.
		
		\item \emph{Linear termination equivalence}: there is a $\tofs$ normalizing evaluation $\deriv$ from $\tm$ iff there 
is a $\tovsubvals$ normalizing evaluation $\derivp$ from $\tm$. Moreover, $\size\deriv\leq \sizep\derivp{\ssym\msym} 
\leq 2\size\deriv$.	
		
		\item \label{pappendix:props-of-tofs-upto} \emph{Strong bisimulation}:
		on light terms $\eqstruct$ is a strong bisimulation with respect to $\tofs$.
	\end{enumerate}
\end{proposition}

\begin{proof}\hfill
	\begin{enumerate}
		\item 
		Since the two calculi share the same definitions of open evaluation contexts $\weakctx$ and strong evaluation 
contexts $\strongctx$, the only interesting cases are the base ones, the other ones follow immediately from the \ih 
%and from the good rewriting properties of the strong bisimulation $\equiv$ (\Cref{prop:strong-bisimulation}, \Cref{cor:eqstruct-post-and-term}).
		\begin{itemize}
			\item \emph{Value} step, \ie $\tm = \sctxp{\la{\var}\tmthree} \sctxtwop{\val} \rtobabs 
\sctxp{\sctxtwop{{\tmthree}\isub{\var}{\val}}} = \tmtwo$.
			Then, $\tm = \sctxp{\la{\var}\tmthree} \sctxtwop{\val} \rtom \sctxp{\tmthree\esub{\var}{\sctxtwop{\val}}} \rtoe 
\sctxp{\sctxtwop{{\tmthree}\isub{\var}{\val}}} = \tmtwo$ and hence 
$1$ $\tobetavs$-step in the fireball calculus is simulated by $1$ $\toms$-step and $1$ $\toes$-step in the VSC. 
		
			\item \emph{Inert} setp, \ie $\tm = \sctxp{\la{\var}\tmthree} {\itm} \rtoin \sctxp{{\tmthree}\esub{\var}{\itm}} = 
\tmtwo$.
			Then, $\tm = \sctxp{\la{\var}\tmthree} \itm \rtom \sctxp{\tmthree\esub{\var}{\itm}}  = \tmtwo$ and hence $1$ 
$\toins$-step in the fireball calculus is simulated by $1$ $\toms$-step in the VSC.
		\end{itemize}
		\item $\Leftarrow:$ By induction on the definition of strong fireball:
			\begin{itemize}
				\item \emph{Strong inert, variable}; \ie, $\tm = \var$: Trivial.
				
				\item \emph{Strong inert, application}; \ie, $\tm = \sitm \sfire$: By \ih, both $\sitm$ and $\sfire$ are in 
$\tofs$-normal form. Moreover, note that the strong inert term $\sitm$ is not a $\lambda$-abstraction in a substitution 
context ---by \reflemma{shape-of-strong-fireballs}---, and so $\tm$ is in $\tofs$-normal form as well.
				
				\item \emph{Strong inert, $\mathsf{ES}$}: \ie, $\tm = \sitm \esub{\var}{\sitmtwo}$: By \ih, both $\sitm$ and 
$\sitmtwo$ are in $\tofs$-normal form. Then $\tm$ is in $\tofs$-normal form as well.
				
				\item \emph{Strong value}: \ie, $\tm = \la{\var}{\sfire}$: By \ih, $\sfire$ is in $\tofs$-normal form. Then so 
is $\tm$.
				
				\item \emph{Strong fireball, $\mathsf{ES}$}: \ie, $\tm = \sfire \esub{\var}{\sitm}$: By \ih, both $\sfire$ and 
$\sitm$ are in $\tofs$-normal form. Then so is $\tm$.
				
			\end{itemize}
		
		$\Rightarrow:$ By induction on the definition of the term $\tm$:
			\begin{itemize}
				\item \emph{Variable}: Trivial.
				
				\item \emph{$\lambda$-abstraction}; \ie, $\tm = \la{\var}{\tmtwo}$: By \ih, $\tmtwo$ is a strong fireball. Then 
so is $\tm$.
				
				\item \emph{Application}; \ie, $\tm = \tmtwo \tmthree$: By \ih, both $\tmtwo$ and $\tmthree$ are strong 
fireballs. Moreover, note that both $\tmtwo$ and $\tmthree$ are either a strong inert term or a value fireball ---by 
\reflemma{shape-of-strong-fireballs}---, and that $\tmtwo$ cannot be a value fireball or otherwise $\tm$ is either not 
in $\rtobv$-normal form or $\rtoin$-normal form ---absurd. Thus, $\tmtwo$ is a strong inert term and then $\tm$ is a 
strong fireball.
				
				\item \emph{$\mathsf{ES}$}; \ie, $\tm = \tmtwo \esub{\var}{\tmthree}$: By \ih, both $\tmtwo$ and $\tmthree$ are 
strong fireballs. Note that $\tmthree$ has to be a strong inert term ---by \reflemma{shape-of-strong-fireballs} and the 
fact that explicit substitutions only contain inert terms---, and so $\tm$ is a strong fireball.
				
			\end{itemize}
		
		\item 
		
		By straightforward inspection of the reduction rules, it easy to see that $\tofs$ is orthogonal (since we are 
restricted to light terms) and hence diamond.
		
		\item Similar to the proof of \cite[Corollary 13]{DBLP:conf/aplas/AccattoliG16}, using 
\refpoint{props-of-tofs-simulation}.
		\item Analogous to the proof of \refprop{strong-bisimulation}.
		\qedhere
	\end{enumerate}
\end{proof}


==> proofs/open/open-type_size_exists.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	By induction on the definition of inert term.
	
	\begin{itemize}
				\item \emph{Variable}, \ie $\tm = \var$. Then $\tderiv$ is a $\ruleManyVar$ rule with $n$ premises $\tderiv_i$ for 
$i\in\set{1,\ldots n}$, which are all axioms. If 
$\imtypetwo = \mset{\inltype_1,\ldots, \inltype_n}$ then the derivation $\concl{\tderivtwo}{\typctxtwo}{\tm}{\imtypetwo}$ for 
the statement is made out of $n$ axioms of types $\inltype_1,\ldots, \inltype_n$ over a $\ruleManyVar$ rule and $\typctxtwo$ 
is simply $\imtypetwo$, so that $\sizectx{\typctxtwo} = \sizetyp{\imtypetwo}$. Then $\tderiv \tderiveq \tderivtwo$.
		

		%%%%%%%%%%%%%%%%%
		\item \emph{Inert application}, \ie $\tm = \itm \fire$ (which is inert). Then $\tderiv$ has the following form. 
		\begin{equation*}
		\tderiv \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctx_{\itm} \vdash \itm \hastype \mset{\larrow{\mtypethree}{\imtype}}}
		\hypo{}
		\ellipsis{$\tderiv_{\fire}$}{\typctx_{\fire} \vdash \fire \hastype \mtypethree}
		\infer2[\footnotesize$\ruleAp$]{\typctx_{\itm}\mplus\typctx_{\fire} \vdash \itm\fire \hastype \imtype}
		\end{prooftree}
		\end{equation*}
		\ben{Since $\tderiv$ is inert, $\typctx_{\itm}$ are $\typctx_{\fire}$ inert, and by the spreading of inertness (\reflemma{spread-inert}), $\mset{\larrow{\mtypethree}{\imtype}}$ is inert. Then $\tderiv_{\itm}$ is inert, and $\mtypethree$ is a ground multi type. Then $\mset{\larrow{\mtypethree}{\imtypetwo}}$ is also inert.}
By \ih, there is a derivation 
$\concl{\tderivtwo_{\itm}}{\typctxtwo_{\itm}}{\itm}{\mset{\larrow{\mtypethree}{\imtypetwo}}}$ such that 
$\tderivtwo_{\itm} \tderiveq \tderiv_{\itm}$.
		We have the following derivation $\tderivtwo$:
		\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo_{\itm}$}{\typctxtwo_{\itm} \vdash \itm \hastype \mset{\larrow{\mtypethree}{\imtypetwo}}}
		\hypo{}
		\ellipsis{$\tderiv_{\fire}$}{\typctx_{\fire} \vdash \fire \hastype \mtypethree}
		\infer2[\footnotesize$\ruleAp$]{\typctxtwo_{\itm}\mplus\typctx_{\fire} \vdash \itm\fire \hastype \imtypetwo}
		\end{prooftree}
		\end{equation*}
		Clearly, $\tderiv \tderiveq \tderivtwo$.
		
		%%%%%%%%%%%%%%%%%%%%%
		\item \emph{Explicit substitution on inert}, \ie $\tm = \itm \esub{\var}{\itmtwo}$.
		Then $\tderiv$ has the following form. 
		\begin{equation*}
		\tderiv \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctx_{\itm}, \var\hastype\mtypetwo \vdash \itm \hastype \imtype}
		\hypo{}
		\ellipsis{$\tderiv_{\itmtwo}$}{\typctx_{\itmtwo} \vdash \itmtwo \hastype \mtypetwo}
		\infer2[\footnotesize$\ruleES$]{\typctx_{\itm} \mplus \typctx_{\itmtwo} \vdash \itm \esub{\var}{\itmtwo} 
\hastype \imtype}
		\end{prooftree}
		\end{equation*}
		with $\typctx = \typctx_{\itm} \mplus \typctx_{\itmtwo}$. \ben{Since $\tderiv$ is inert, $\typctx_{\itm}$ and $\typctx_{\itmtwo}$ are inert, and by the spreading of inertness (\reflemma{spread-inert}), $\mtypetwo$ is inert. Then $\tderiv_{\itm}$ is inert.}
		By \ih, there is a derivation $\concl{\tderivtwo_{\itm}}{\typctxtwo_{\itm}, 
\var\hastype\mtypethree}{\itm}{\imtypetwo}$ such that $\tderivtwo_{\itm} \tderiveq \tderiv_{\itm}$. By 
\reflemma{skel-equiv-properties}, $\mtypethree$ has the same cardinality of the type $\mtypetwo$ given by 
$\tderiv_{\itm}$ to $\var$, which is also the same type given by $\tderiv_{\itmtwo}$ to $\itmtwo$. We can then apply 
the \ih and obtain a derivation $\concl{\tderivtwo_{\itmtwo}}{\typctxtwo_{\itmtwo}}{\itmtwo}{\mtypethree}$ such that 
$\tderivtwo_{\itmtwo} \tderiveq \tderiv_{\itmtwo}$.
		We have the following derivation $\tderivtwo$:
		\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo_{\itm}$}{\typctxtwo_{\itm}, \var\hastype\mtypethree \vdash \itm \hastype \imtypetwo}
		\hypo{}
		\ellipsis{$\tderivtwo_{\itmtwo}$}{\typctxtwo_{\itmtwo} \vdash \itmtwo \hastype \mtypethree}
		\infer2[\footnotesize$\ruleES$]{\typctxtwo_{\itm} \mplus \typctxtwo_{\itmtwo} \vdash \itm \esub{\var}{\itmtwo} 
\hastype \imtypetwo}
		\end{prooftree}
		\end{equation*}
Clearly, $\tderiv \tderiveq \tderivtwo$. \qedhere
	\end{itemize}	
\end{proof}


==> proofs/open/open-type_size_exists2.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	By mutual induction on the definition of inert term and fireball.	
	\begin{itemize}
				\item \emph{Variable}, \ie $\tm = \var$ (which is inert). Then both $\tderiv$ and $\tderivtwo$ are given by a $\ruleManyVar$ rule with $n_\tderiv$ and $n_\tderivtwo$ premises, which are all axioms. Since the multiplicative size of axioms is $0$, we have $\sizem{\tderiv} = 0 = \sizem{\tderivtwo}$. 		

		%%%%%%%%%%%%%%%%%
		\item \emph{Inert application}, \ie $\tm = \itm \fire$ (which is inert). Then $\tderiv$ has the following form. 
		\begin{equation*}
		\tderiv \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctx_{\itm} \vdash \itm \hastype \mset{\larrow{\mtypetwo}{\mtype}}}
		\hypo{}
		\ellipsis{$\tderiv_{\fire}$}{\typctx_{\fire} \vdash \fire \hastype \mtypetwo}
		\infer2[\footnotesize$\ruleAp$]{\typctx_{\itm}\mplus\typctx_{\fire} \vdash \itm\fire \hastype \mtype}
		\end{prooftree}
		\end{equation*}
		\ben{Since $\tderiv$ is inert, $\typctx_{\itm}$ are $\typctx_{\fire}$ inert, and by the spreading of inertness (\reflemma{spread-inert}), $\mset{\larrow{\mtypetwo}{\mtype}}$ is inert. Then $\tderiv_{\itm}$ is inert, and $\mtypetwo$ is a ground multi type. Then $\tderiv_{\fire}$ is tight.}
		Similarly, $\tderivtwo$ ends with a $\ruleAp$ rule, its premise $\tderivtwo_\itm$ is inert and its premise $\tderivtwo_\fire$ is tight. Then we can apply the \ih (point 1) to $\tderiv_\itm$ and $\tderivtwo_\itm$, and the \ih (point 2) to $\tderiv_\fire$ and $\tderivtwo_\fire$, obtaining $\sizem\tderiv = \sizem{\tderiv_{\itm}}+ \sizem{\tderiv_{\fire}} + 1 =_{\ih} \sizem{\tderivtwo_{\itm}}+ \sizem{\tderivtwo_{\fire}} + 1 = \sizem\tderivtwo$.
		
		%%%%%%%%%%%%%%%%%%%%%
		\item \emph{Explicit substitution on inert}, \ie $\tm = \itm \esub{\var}{\itmtwo}$ (which is inert).
		Then necessarily
		\begin{equation*}
		\tderiv = 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctxtwo, \var \hastype \mtypetwo \vdash \itm \hastype \mtype}
		\hypo{}
		\ellipsis{$\tderiv_{\itmtwo}$}{\typctxthree \vdash \itmtwo \hastype \mtypetwo}
		\infer2[\footnotesize$\ruleES$]{\tyjp{}{\itm \esub{\var}{\itmtwo}}{\typctxtwo \mplus \typctxthree}{\mtype}}
		\end{prooftree}
		\end{equation*}
		where $\typctx = \typctxtwo \mplus \typctxthree$. \ben{Since $\tderiv$ is inert, $\typctxthree$ is inert, and by the 
spreading of inertness (\reflemma{spread-inert}) $\mtypetwo$ is inert.} Similarly, $\tderivtwo$ ends with a $\ruleES$ rule, and its two premises $\tderivtwo_\itm$ and $\tderivtwo_{\itmtwo}$ are inert. Then $\sizem\tderiv = \sizem{\tderiv_{\itm}}+ \sizem{\tderiv_{\itmtwo}} =_{\ih} \sizem{\tderivtwo_{\itm}}+ \sizem{\tderivtwo_{\itmtwo}} = \sizem\tderivtwo$.

		%%%%%%%%%%%%%%%%%		
		\item \emph{Abstraction}, \ie $\fire = \la{\var}{\firetwo}$. 
		Both $\tderiv$ and $\tderivtwo$ are tight, that is, they type $\fire$ with a ground multi type. Since they also have to end with a rule $\ruleManyVal$ whose  premises end with a $\ruleFun$ rule, which does not assign a ground type, the only possibility is that both $\ruleManyVal$ rules have $0$ premises and they type $\fire$ with $\zero$. Then $\sizem{\tderiv} = 0 = \sizem{\tderivtwo}$.
						
		
		%%%%%%%%%%%%%%%%%%%%%%%
		\item \emph{Explicit substitution on fireball}, \ie $\tm = \fire \esub{\var}{\itm}$. Since $\tderiv$ is tight, it 
has the following shape.
		\begin{equation*}
		\tderiv = 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\fire}$}{\typctxtwo, \var \hastype \mtypetwo \vdash \fire \hastype \gmtype}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctxthree \vdash \itm \hastype \mtypetwo}
		\infer2[\footnotesize$\ruleES$]{\tyjp{}{\fire \esub{\var}{\itm}}{\typctxtwo \mplus \typctxthree}{\gmtype}}
		\end{prooftree}
		\end{equation*}
		where $\typctx = \typctxtwo \mplus \typctxthree$. \ben{Since $\tderiv$ is tight, $\typctxthree$ is inert, and by the 
spreading of inertness (\reflemma{spread-inert}) $\mtypetwo$ is inert.}
Similarly, $\tderivtwo$ ends with a $\ruleES$ rule, its premise $\tderivtwo_\itm$ is inert and its premise $\tderivtwo_\fire$ is tight. Then we can apply the \ih (point 1) to $\tderiv_\itm$ and $\tderivtwo_\itm$, and the \ih (point 2) to $\tderiv_\fire$ and $\tderivtwo_\fire$, obtaining $\sizem\tderiv = \sizem{\tderiv_{\fire}} + \sizem{\tderiv_{\itm}}=_{\ih} \sizem{\tderivtwo_{\fire}} + \sizem{\tderivtwo_{\itm}}= \sizem\tderivtwo$.
\qedhere
	\end{itemize}	
\end{proof}


==> proofs/open/open-type_size_forall.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	By mutual induction on the definition of inert term and fireball.
	Note that the statement for the former implies the one for the latter, because if $\tderiv$ is tight then $\imtype$ is a ground multi type, for which $\sizetyp{\imtype} = 0$. Hence for inert terms it is enough to 
	prove \refpoint{open-types-bound-normal-derivations-inert}.
	Cases: 
	\begin{itemize}
		\item \emph{Variable}, \ie~$\tm = \var$ (which is inert). So, necessarily, for some set of indices $I$,
		\begin{equation*}
		\tderiv = 
		\begin{prooftree}
		\infer0[\footnotesize$\ruleAx$]{\tyjp{}{\var}{\var \hastype \mset{\inltype_j}}{\inltype_j}}
		\delims{\left[}{\right]_{\jJ}}
		\infer1[\footnotesize$\ruleManyVar$]{\tyjp{}{\var}{\var \hastype \imtype}{\imtype}}
		\end{prooftree}
		\end{equation*}
		where $\imtype = \mset{\inltype_j}_{\jJ}$ and $\typctx = \var \hastype \imtype$.
		Since $\sizem{\tderiv} = 0$ and $\sizetyp{\imtype} = \sizectx{\typctx}$,
		then $\sizem{\tderiv} = 0 = \sizectx{\typctx}- \sizetyp{\imtype}$.
				
		\item \emph{Application}, \ie~$\tm = \itm \fire$ (which is inert). 
		Then necessarily
		\begin{equation*}
		\tderiv = 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctxtwo \vdash \itm \hastype \mult{\larrow{\mtypetwo}{\imtype}}}
		\hypo{}
		\ellipsis{$\tderiv_{\fire}$}{\typctxthree \vdash \fire \hastype\mtypetwo}
		\infer2[\footnotesize$\ruleApp$]{\tyjp{}{\itm \fire}{\typctxtwo \mplus \typctxthree}{\imtype}}
		\end{prooftree}
		\end{equation*}
		where $\typctx = \typctxtwo \mplus \typctxthree$. \ben{Since $\tderiv$ is inert, $\typctxtwo$ is inert, and by the 
spreading of inertness (\reflemma{spread-inert}) $\mult{\larrow{\mtypetwo}{\imtype}}$ is inert. Therefore, $\mtypetwo$ is a ground multi type and $\tderiv_{\fire}$ is tight}.
		By \ih (point 1 for $\tderiv_{\itm}$, point 2 for $\tderiv_{\fire}$), $\sizem{\tderiv_{\itm}} = \sizectx{\typctxtwo} 
- \sizetyp{\mset{\larrow{\mtypetwo}{\imtype}}} = \sizectx{\typctxtwo} - \sizetyp{\imtype} -1$, because ground multi types have size $0$,  and $\sizem{\tderiv_{\fire}} = 
\sizectx{\typctxthree}$. 
		Therefore, 
		\[\begin{array}{rcl}
		\sizem{\tderiv} & = & \sizem{\tderiv_{\itm}} + \sizem{\tderiv_{\fire}} + 1 
		\\
		& =_{\ih} &\sizectx{\typctxtwo} - \sizetyp{\imtype} -1+ \sizem{\tderiv_{\fire}} + 1  
		\\
		& = &\sizectx{\typctxtwo} - \sizetyp{\imtype}+ \sizem{\tderiv_{\fire}}   
		\\
		& =_{\ih} & \sizectx{\typctxtwo} - \sizetyp{\imtype}+ \sizectx{\typctxthree}
		\\
		& = & \sizectx{\typctx} - \sizetyp{\imtype}.
		\end{array}\]
		
		\item \emph{Explicit substitution on inert}, \ie $\tm = \itm \esub{\var}{\itmtwo}$ (which is inert).
		Then necessarily
		\begin{equation*}
		\tderiv = 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctxtwo, \var \hastype \mtypetwo \vdash \itm \hastype \imtype}
		\hypo{}
		\ellipsis{$\tderiv_{\itmtwo}$}{\typctxthree \vdash \itmtwo \hastype \mtypetwo}
		\infer2[\footnotesize$\ruleES$]{\tyjp{}{\itm \esub{\var}{\itmtwo}}{\typctxtwo \mplus \typctxthree}{\imtype}}
		\end{prooftree}
		\end{equation*}
		where $\typctx = \typctxtwo \mplus \typctxthree$. \ben{Since $\tderiv$ is inert, $\typctxthree$ is inert, and by the 
spreading of inertness (\reflemma{spread-inert}) $\mtypetwo$ is inert.} Therefore both $\tderiv_{\itm}$ and 
$\tderiv_{\itmtwo}$ are inert. 
		By \ih (point 1), $\sizem{\tderiv_{\itm}} = \sizectx{\typctxtwo} + \sizetyp{\mtypetwo} - \sizetyp{\imtype}$ and $ 
\sizem{\tderiv_{\itmtwo}} = \sizectx{\typctxthree} - \sizetyp{\mtypetwo}$. 
		So, 
		\[\begin{array}{rcl}
		\sizem{\tderiv} & = & \sizem{\tderiv_{\itm}} + \sizem{\tderiv_{\itmtwo}}
		\\
		& =_{\ih} & \sizectx{\typctxtwo} + \sizetyp{\mtypetwo} - \sizetyp{\imtype} + \sizem{\tderiv_{\itmtwo}}
		\\
		& =_{\ih} & \sizectx{\typctxtwo} + \sizetyp{\mtypetwo} - \sizetyp{\imtype} + \sizectx{\typctxthree} - 
\sizetyp{\mtypetwo}
		\\
		& = & \sizectx{\typctxtwo} + \sizectx{\typctxthree} - \sizetyp{\imtype}
		\\
		& = & \sizectx{\typctx} - \sizetyp{\imtype}.
		\end{array}\]
		
		\item \emph{Explicit substitution on fireball}, \ie $\tm = \fire \esub{\var}{\itm}$. Since $\tderiv$ is tight, it 
has the following shape.
		\begin{equation*}
		\tderiv = 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\fire}$}{\typctxtwo, \var \hastype \mtypetwo \vdash \fire \hastype \gmtype}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctxthree \vdash \itm \hastype \mtypetwo}
		\infer2[\footnotesize$\ruleES$]{\tyjp{}{\fire \esub{\var}{\itm}}{\typctxtwo \mplus \typctxthree}{\gmtype}}
		\end{prooftree}
		\end{equation*}
		where $\typctx = \typctxtwo \mplus \typctxthree$. \ben{Since $\tderiv$ is tight, $\typctxthree$ is inert, and by the 
spreading of inertness (\reflemma{spread-inert}) $\mtypetwo$ is inert.}
		By \ih (point 1 for $\tderiv_{\itm}$, point 2 for $\tderiv_{\fire}$), $\sizem{\tderiv_{\fire}} = \sizectx{\typctxtwo} + \sizetyp{\mtypetwo} $  and $ \sizem{\tderiv_{\itm}} = 
\sizectx{\typctxthree}-\sizetyp{\mtypetwo}$. 
		Therefore, 
		\[\begin{array}{rcl}
		\size{\tderiv} & = & \sizem{\tderiv_{\fire}} + \sizem{\tderiv_{\itm}}
		\\
		& =_{\ih} & \sizectx{\typctxtwo} + \sizetyp{\mtypetwo} + \sizem{\tderiv_{\itm}}
		\\
		& =_{\ih} & 
		\sizectx{\typctxtwo} + \sizetyp{\mtypetwo} + \sizectx{\typctxthree} - \sizetyp{\mtypetwo}
		\\
		& = & \sizectx{\typctxtwo} + \sizectx{\typctxthree} .
		\\
		& = & \sizectx{\typctx}.
		\end{array}\]
		
		\item \emph{Abstraction}, \ie $\tm = \la{\var}{\tmtwo}$. Since 	$\tderiv$ is tight, it types $\fire$ with a ground multi type. Now, $\tderiv$ also has to end with a rule $\ruleManyVal$, whose premises end with a $\ruleFun$ rule. But $\ruleFun$ does not assign a ground type---the only possibility is that rule $\ruleManyVal$ has $0$ premises and that $\tderiv$ types $\fire$ with $\zero$, as follows.
		\begin{equation*}
		\begin{prooftree}
		\infer0[\footnotesize$\ruleManyVal$]{\vdash \la{\var}\fire \hastype \zero}		
		\end{prooftree}
		\end{equation*}
		Then $\typctx$ is empty and $\sizem\tderiv = 0 = \sizectx\typctx$.
		\qedhere
	\end{itemize}
\end{proof}

